A Study of Revenue Cost Dynamics in Large Data Centers: A Factorial Design Approach

Revenue optimization of large data centers is an open and challenging problem. The intricacy of the problem is due to the presence of too many parameters posing as costs or investment. This paper proposes a model to optimize the revenue in cloud data center and analyzes the model, revenue and different investment or cost commitments of organizations investing in data centers. The model uses the Cobb-Douglas production function to quantify the boundaries and the most significant factors to generate the revenue. The dynamics between revenue and cost is explored by designing an experiment (DoE) which is an interpretation of revenue as function of cost/investment as factors with different levels/fluctuations. Optimal elasticities associated with these factors of the model for maximum revenue are computed and verified . The model response is interpreted in light of the business scenario of data centers.

==> authorinformation.tex <==

\begin{IEEEbiographynophoto}{Gambhire Swati Sampatrao}
Ms Gambhire Swati Sampatrao is a B.E and Mtech in Computer science and engineering.She has 7yrs of teaching experience in various institutions.Her research areas are Cloud Computing,Optimization techniques and Artificial Neural Networks.
\end{IEEEbiographynophoto}


\begin{IEEEbiographynophoto}{Snehanshu Saha}
Biography text here.
\end{IEEEbiographynophoto}



\begin{IEEEbiographynophoto}{Sai Prasanna}
Ms Sai Prasanna is a B.E and M.tech in Computer science and engineering.She has 2yrs of teaching experience in various institutions.Her research areas are Cloud Computing and Artificial Neural Networks.
\end{IEEEbiographynophoto}
